Analysis of Periodic Feedback Shift Registers

This paper develops methods for analyzing periodic orbits of states of linear feedback shift registers with periodic coefficients and estimating their lengths. These shift registers are among the simplest nonlinear feedback shift registers (FSRs) whose orbit lengths can be determined by feasible computation. In general such a problem for nonlinear FSRs involves infeasible computation. The dynamical systems whose model includes such FSRs are termed as Periodic Finite State systems (PFSS). This paper advances theory of such dynamical systems. Due to the finite field valued coefficients, the theory of such systems turns out to be radically different from that of linear continuous or discrete time periodic systems with real coefficients well known in literature. A special finite field version of the Floquet theory of such periodic systems is developed and the structure of trajectories of the PFSS is analyzed through that of a shift invariant linear system after Floquet transformation. The concept of extension of a dynamical system is proposed for such systems whenever the equivalent shift invariant system can be obtained over an extension field.

==> sec6NumExamples.tex <==
\section{Numerical Examples}
In this section, some numerical examples have been discussed to validate the theory developed. First we discuss about a PFSS which has a Floquet transform and look at how the solutions are computed using Floquet theory. The second example discusses about a PFSS which does not allow a Floquet transform. 
\subsection{PFSS with Floquet transform}
Consider a system evolving over $\ff_2^2$ with $N=2$  \begin{equation}
    A(0) = \begin{bmatrix} 1 & 1 \\ 0 & 1\end{bmatrix} \hspace{0.2in}
    A(1) = \begin{bmatrix} 0& 1 \\ 1 & 0\end{bmatrix}  \hspace{0.2in}
\end{equation}
\[
    \Phi = A(1)A(0) =  \begin{bmatrix} 0 & 1 \\ 1 & 1 
    \end{bmatrix}
\]
We see that $\Phi$ has a square root ($\tA$) 
\[
\tA = \begin{bmatrix} 1 & 1 \\ 1 & 0\end{bmatrix}
\]
The Floquet transform matrices
\begin{align*}
         \hspace{0.2in}
         P(0) = \begin{bmatrix} 1 & 0 \\ 0 & 1\end{bmatrix} \hspace{0.2in} 
         P(1) = \begin{bmatrix} 1 & 0 \\ 1 & 1\end{bmatrix}
\end{align*}
and the equivalent LFSS 
\beq
\tx(k+1) =  \begin{bmatrix} 1 & 1 \\ 1 & 0\end{bmatrix} \tx(k)
\eeq 
Note that $\kmA = \{0\}$. So, all initial condition other than $0$ have a orbit length which is a multiple of $N$. From the linear theory, we note that $\tA$ has orbit of length $3$ for any non-zero $\tx(0)$. Since $P(0) = I$, any non-zero $x(0)$ will have orbit of length $lcm(3,2) = 6$. We see the following state evolution for the different initial condition which corroborates the theory
\begin{itemize}
    \item $\begin{bmatrix} 0 \\ 1 \end{bmatrix} \xrightarrow{A(0)} \begin{bmatrix} 1 \\ 1 \end{bmatrix} \xrightarrow{A(1)} \begin{bmatrix} 1 \\ 1 \end{bmatrix} \xrightarrow{A(0)} \begin{bmatrix} 0 \\ 1  \end{bmatrix} \xrightarrow{A(1)} \begin{bmatrix} 1 \\ 0 \end{bmatrix} \xrightarrow{A(0)} \begin{bmatrix} 1 \\ 0 \end{bmatrix} \xrightarrow{A(1)} \begin{bmatrix} 0 \\ 1 \end{bmatrix} \xrightarrow{A(0)}\cdots \cdots$
    \item $ \begin{bmatrix} 1 \\ 1 \end{bmatrix} \xrightarrow{A(0)} \begin{bmatrix} 0 \\ 1  \end{bmatrix} \xrightarrow{A(1)} \begin{bmatrix} 1 \\ 0 \end{bmatrix} \xrightarrow{A(0)} \begin{bmatrix} 1 \\ 0 \end{bmatrix} \xrightarrow{A(1)} \begin{bmatrix} 0 \\ 1 \end{bmatrix}\xrightarrow{A(0)} \begin{bmatrix} 1 \\ 1 \end{bmatrix} \xrightarrow{A(1)} \begin{bmatrix} 1 \\ 1 \end{bmatrix} \xrightarrow{A(0)} \cdots \cdots$
    \item $\begin{bmatrix} 1 \\ 0 \end{bmatrix} \xrightarrow{A(0)} \begin{bmatrix} 1 \\ 0 \end{bmatrix} \xrightarrow{A(1)} \begin{bmatrix} 0 \\ 1 \end{bmatrix}\xrightarrow{A(0)} \begin{bmatrix} 1 \\ 1 \end{bmatrix} \xrightarrow{A(1)} \begin{bmatrix} 1 \\ 1 \end{bmatrix} \xrightarrow{A(0)}\begin{bmatrix} 0 \\ 1  \end{bmatrix} \xrightarrow{A(1)} \begin{bmatrix} 1 \\ 0 \end{bmatrix} \xrightarrow{A(0)} \cdots \cdots$
\end{itemize}
So all orbits of the PFSS are given by 
\[
\Sigma_{PFSS} =\{ 1[1] + 3[6] \}
\]
\subsection{PFSS without Floquet transform}
Consider a PFSS over $\ff_2^2$ with period $2$
\begin{equation}
    A(0) = \begin{bmatrix} 1 & 1 \\ 1 & 0\end{bmatrix} \hspace{0.2in}
    A(1) = \begin{bmatrix} 1& 0 \\ 1 & 1\end{bmatrix}  \hspace{0.2in}
\end{equation}
\[
    \Phi = A(1)A(0) =  \begin{bmatrix} 1 & 1 \\ 0 & 1 
    \end{bmatrix}
\]
As discussed before, this matrix $\Phi$ does not have a square root over any rings of matrices defined over field of characteristic $2$. This system does not have Floquet transfrom. Still from the analysis done in section \ref{sec:SolutionsPFSS}, we know that any solution $x(k)$ not completely in $\kmA$ will have a period which is a multiple of $N$. $\kmA$ is computed to be 
\[
\kmA = \{ \begin{bmatrix} 0 \\ 0 \end{bmatrix}, \begin{bmatrix} 1 \\ 0 \end{bmatrix} \}
\]
$x(0) = 0$ is a fixed point. For non-zero initial conditions. we have the following state evolution
\begin{enumerate}
    \item $\begin{bmatrix} 0 \\ 1 \end{bmatrix} \xrightarrow{A(0)} \begin{bmatrix} 1 \\ 0 \end{bmatrix} \xrightarrow{A(1)} \begin{bmatrix} 1 \\ 1 \end{bmatrix} \xrightarrow{A(0)} \begin{bmatrix} 0 \\ 1  \end{bmatrix} \xrightarrow{A(1)} \begin{bmatrix} 0 \\ 0 \end{bmatrix} \xrightarrow{A(0)} \cdots \cdots$
    \item $ \begin{bmatrix} 1 \\ 1 \end{bmatrix} \xrightarrow{A(0)} \begin{bmatrix} 0 \\ 1  \end{bmatrix} \xrightarrow{A(1)} \begin{bmatrix} 0 \\ 1 \end{bmatrix} \xrightarrow{A(0)} \begin{bmatrix} 1 \\ 0 \end{bmatrix} \xrightarrow{A(1)} \begin{bmatrix} 1 \\ 1 \end{bmatrix} \xrightarrow{A(0)} \cdots \cdots$
    \item $\begin{bmatrix} 1 \\ 0 \end{bmatrix} \xrightarrow{A(0)} \begin{bmatrix} 1 \\ 1 \end{bmatrix} \xrightarrow{A(1)} \begin{bmatrix} 1 \\ 0 \end{bmatrix} \xrightarrow{A(0)} \cdots \cdots$
\end{enumerate}
We see that even though the initial condition $\begin{bmatrix} 1 \\ 0 \end{bmatrix} \in \kmA$, the next state goes out of $\kmA$. So by result \ref{thm:CoprimeT}, the orbit length is $2$ which is a multiple of $N$. The other two initial conditions too have a orbit length of $4$ which is a multiple of $2$ again. 
